Topological properties of real algebraic varieties: du c\^ot\'e de chez Rokhlin

The survey gives an overview of the achievements in topology of real algebraic varieties in the direction initiated in the early 70th by V.I.Arnold and V.A.Rokhlin. We make an attempt to systematize the principal results in the subject. After an exposition of general tools and results, special attention is paid to surfaces and curves on surfaces.

==> f-4s-nc.tex <==
%Version: Alex Degtyarev 28/07/98  16:48:53
%Format: plain

\newdimen\hstep
\newdimen\vstep
{\catcode`\@=11
\global\hstep5\p@
\global\vstep4\p@
\gdef\nwdotline#1{\vbox to\z@{\vss\hbox to\z@{\hss%
 \count@=#1 \dimen@=\z@ \setbox\z@\hbox to\z@{\hss.\hss}%
 \loop \raise\dimen@\copy\z@\kern-\hstep
   \advance\count@\m@ne\advance\dimen@\vstep
   \ifnum\count@>0\repeat
 \kern#1\hstep
}}}
\gdef\nedotline#1{\vbox to\z@{\vss\hbox to\z@{%
 \count@=#1 \dimen@=\z@ \setbox\z@\hbox to\z@{\hss.\hss}%
 \loop \raise\dimen@\copy\z@\kern\hstep
   \advance\count@\m@ne\advance\dimen@\vstep
   \ifnum\count@>0\repeat
\hss}}}
}

\def\mbox#1{\hbox to6pt{\hss$#1$\hss}}
\def\.{\mbox{\bullet}}
\def\,{\mbox{\circ}}
\def\*{\mbox{*}}
\def\d{\mbox{\cdot}\kern-6pt\mbox{\circ}}
\hbox to\hsize{\hss\vbox{\offinterlineskip
\ialign{\hss\eightrm#\quad\vrule&&\strut\hbox to15pt{\eightrm\hss#\hss}\cr
$a$&&&&&&&&&&&&&&&&&\cr
&&&&&&&&&&&&&&&&&\cr
0&&\*&&&&&&&&\*&&&&&&&&\*\cr
1&\.&&\.&&&&&&\.&&\.&&&&&&\.&&\.\cr
2&&\.\*&&\.&&\*&&\.&&\.\*&&\.&&\*&&\.&&\.\*&\cr
3&&&\.&&\.&&\.&&\.&&\.&&\.&&\.&&\.&\cr
4&&&&\.&&\.&&\.&&\.\*&&\.&&\.&&\.&\cr
5&&&&&\.&&\.&&\.&&\.&&\.&&\.&\cr
6&&&&&&\.&&\.&&\.\*&&\.&&\.&\cr
7&&&&&&&\.&&\.&&\.&&\.&\nwdotline{19}\cr
8&&&&&&&&\.&&\.\d&&\.&\cr
9&&&&&&&&&\.&&\.&\cr
10&&&&&&&&&&\.&\cr
\noalign{\hrule}
&1&2&3&4&5&6&7&8&9&10&11&12&13&14&15&16&17&18&19&&&r\cr}}\hss}
%\noalign{%
\figure[Table]\label{4surf.nc}
Noncontractible quartic surfaces in $\RP^3$
\endfigure
\bigskip\bigskip
\hbox to\hsize{\hss\vbox{\offinterlineskip
\ialign{\hss\eightrm#\quad\vrule&&\strut\hbox to15pt{\eightrm\hss#\hss}\cr
%}\crcr
$a$&&&&&&&&&&&&&&&&&\cr
&&&&&&&&&&&&&&&&&\cr
2&&\*&&\,&&\*&&\,&&\*&&\,&&\*&&\,&&\*&&\,\cr
3&&&\.&&\.&&\.&&\.&&\.&&\.&&\.&&\.&&\.\cr
4&&&&\.\,&&\.\*&&\.\,&&\.\*&&\.\,&&\.\*&&\.\,&&\.\*\cr
5&&&&&\.&&\.&&\.&&\.&&\.&&\.&&\.\cr
6&&&&&&\.&&\.\,&&\.\*&\nwdotline{15}\nedotline{15}&\.\,&&\.\*&&\.\cr
7&&&&&&&\.&&\.&&\.&&\.&&\.\cr
8&&&&&&&&\.\,&&\.&&\.\,&&\.\cr
9&&&&&&&&&\.&&\.&&\.\cr
10&&&&&&&&&&\.\d&&\.\,\cr
11&&&&&&&&&&&\.&&&&&&\cr
\noalign{\hrule}
&1&2&3&4&5&6&7&8&9&10&11&12&13&14&15&16&17&18&19&20&&r\cr}}\hss}
%\noalign{%
\figure[Table]\label{4surf.c}
Contractible quartic surfaces in $\RP^3$
\endfigure
%}\crcr}

\bigskip\eightpoint\noindent
\* and \d\ stand for a surface of type~$\I0$, \, stands for a surface of
type~$\Ihp$, and \. stands for a surface of type~$\II$. The surfaces of
type~$\I0$ denoted by \d\ have $\RX=2S_1$ ($(a,r)=(8,10)$ in
Table~\ref{4surf.nc}) or $\RX=\varnothing$ ($(a,r)=(10,10)$ in
Table~\ref{4surf.c}); the surfaces with $a+r=22$ (the right edge of
Table~\ref{4surf.c}) have $\RX=(r-10)S$; the other surfaces have
$\RX=S_g\+kS$, where $g=\12(22-a-r)$ and $k=\12(r-a)$. The surfaces below
(respectively, above) the dotted lines are (respectively, are not) rigidly
isotopic to their mirror images.
%\end
\endinput

